NUTRIG: Towards an Autonomous Radio Trigger for GRAND

One of the major challenges for large-scale radio surface arrays, such as the Giant Radio Array for Neutrino Detection (GRAND), is the requirement of an autonomous online trigger for radio signals induced by extensive air showers. The NUTRIG project lays the foundations for the development of a pure, efficient, and scalable trigger in the context of GRAND. For this purpose, a GRAND prototype setup of four detection units has been deployed at Nan\c{c}ay, France, which currently serves as the main testing facility for the deployment of this autonomous trigger. This work provides a detailed description of the GRAND@Nan\c{c}ay setup, and a first analysis of background data gathered on site. Initial tests of signal recovery in laboratory conditions are also presented. Finally, near-future plans are outlined to scale NUTRIG to larger pathfinder arrays such as GRANDProto300.

==> ChangeLog <==

2023.02.13	v1	first version.   
2023.04.25	v2	fix "skelecton.tex" to use "\onbehalf{..}" for collaboration. 
2023.06.13	v3	fix typo in "PoStemplate_coll.odt".

